Undetectable Watermarks for Language Models

Recent advances in the capabilities of large language models such as GPT-4 have spurred increasing concern about our ability to detect AI-generated text. Prior works have suggested methods of embedding watermarks in model outputs, by noticeably altering the output distribution. We ask: Is it possible to introduce a watermark without incurring any detectable change to the output distribution? To this end we introduce a cryptographically-inspired notion of undetectable watermarks for language models. That is, watermarks can be detected only with the knowledge of a secret key; without the secret key, it is computationally intractable to distinguish watermarked outputs from those of the original model. In particular, it is impossible for a user to observe any degradation in the quality of the text. Crucially, watermarks should remain undetectable even when the user is allowed to adaptively query the model with arbitrarily chosen prompts. We construct undetectable watermarks based on the existence of one-way functions, a standard assumption in cryptography.

==> 99-old-completeness-proof.tex <==
\begin{theorem}
    For any constant $c$, and any polynomial $\poly(\cdot)$, the simplified watermarking scheme $\calW^s$ with $L = c \cdot \secpar$ is $(2\secpar, L)$-complete, $\frac{1}{\poly(\secpar)}$-sound, and undetectable.
\end{theorem}

\begin{proof}
    \par{\textbf{Soundness.}} 
    By security of the pseudo-random function $F_\sk$, it suffices to prove soundness assuming $F$ is a random oracle.
    Let $(x_1, \ldots, x_n) \in \calT^*$ be some sequence of tokens, let $i \leq n - \secpar$, let $i+1 \leq j \leq n-\secpar$, and let $k_{i,j} = \min\{j+L, n\}$. Let $f$ be a random function. We upper bound the probability that the detector outputs $\true$ in iteration $(i,j)$.

    We break the proof into two cases: $k_{i,j} - j + 1\leq \sqrt{\secpar}$, and $k_{i,j} - j + 1 \geq \sqrt{\secpar}$.
    First, assume that $k_{i,j} - j + 1 \leq \sqrt{\secpar}$. In order for the detector to output $\true$, must have that $c_{i,j} \geq \secpar$, implying that for some $\ell \geq j$, $\ln \frac{1}{1 - F_\sk(r, \ell, x_\ell)} \geq \frac{\sqrt{\secpar}}{2}$. Treating $F$ as a random oracle, observe that for a uniformly random $r \in [0,1]$,
    \[ \Pr_r\left[\ln \frac{1}{1-r} \geq \frac{\sqrt{\secpar}}{2}\right] = \Pr_r\left[r \geq 1 - e^{-\frac{\sqrt{\secpar}}{2}} \right] \leq \negl\]
    By a union bound, the probability that there exists $\ell$ between $j$ and $k_{i,j}$ such that  $\ln \frac{1}{1 - F_\sk(r, \ell, x_\ell)} \geq \sqrt{\secpar}$ is negligible.
    
    Now assume that $k_{i,j} - j + 1 \geq \sqrt{\secpar}$.
    By \Cref{lemma:expected-random-detect} and linearity of expectation, 
    $$E_f\left[\sum_{\ell = j}^{k_{i,j}} \ln \frac{1}{1-f(r,\ell,x_\ell)}\right] = k_{i,j} - j + 1 \leq L$$
    Since we include the counter $j$ in the input to $f$, each term in the sum is independent. Therefore, we can apply a Chernoff bound, letting $X_\ell$ be the random variable taking on the value $\ln \frac{1}{1-f(r,\ell,x_\ell)}$, and letting $\delta$ be the constant such that $(k_{i,j} - j + 1)(1 + \delta) \geq k_{i,j} - j + 1 +  \frac{\secpar}{2}$.\footnote{$\delta$ is a constant because $k_{i,j} - j + 1 \leq L = c \cdot \secpar$}
    $$\Pr \left[ \sum_{\ell=j}^{k_{i,j}} X_\ell \geq (k_{i,j} - j + 1)(1 + \delta)\right] \leq \exp{\frac{-(k_{i,j} - j + 1)\delta^2}{3}} \leq \exp{\frac{-\sqrt{\secpar} \delta^2}{3}} \leq \negl$$
    
    We've shown that in either case, the detector outputs $\true$ on iteration $(i,j)$ with negligble probability. By a union bound over $n^2$, the number of iterations, the probability that the detector outputs $\true$ is negligible.
    % Let $t \geq \frac{1}{2} + \Omega(1)$, and let $\delta$ be a constant such that $t = (1 + \delta) \frac{1}{2}$.\orz{This is all part of the theorem statement, not part of the proof.}
    % For any sequence of tokens $(x_1, \ldots, x_n) \in \calT^*$ and any $i \leq n - \secpar$, for a random function $f$,
    % \begin{align*}
    %     \Pr_f\left[\frac{1}{n-i}\sum_{j=i+1}^n \mathbbm{1}[f((x_1, \hdots, x_{i-1}), j, x) = 1] \geq t \right] &= \Pr \left[\frac{1}{n-i}\sum_{j=i+1}^n X_j \geq t\right]
    % \end{align*}
    % where each $X_j \sim \text{Ber}(\frac{1}{2})$ is a random variable that is equal to 1 if and only if $f((x_1, \hdots, x_{i-1}), j, x) = 1$.
    % Observe that $\E_f\left[\sum_{j=i+1}^n X_j \right] = \frac{n-i}{2}$, which is at least $\frac{\secpar}{2}$. We apply a Chernoff bound to obtain 
    % \[\Pr \left[\frac{1}{n-i}\sum_{j=i+1}^n X_j \geq (1+\delta)\frac{1}{2}\right] \leq \exp{\frac{-\delta^2\secpar}{2(2+\delta)}} \leq \negl\]
    % The probability that the detection algorithm outputs $\true$ given a random function is at most the probability that there exists some $i \leq n-\secpar$ such that $\frac{1}{n-i}\sum_{j=i+1}^n X_j \geq t$. 
    % By a union bound, this probability is at most $(n-1)\negl$, which is negligible.
    % \orz{Should all be made more rigorous. Our correctness bound is going to depend on~$n$, so we can't just assume that~$n\rightarrow \infty$ in the soundness, we need actual bounds for everything.}
    % \mir{This is true for all $n$. The detector as written can only output true if $n - i\geq \secpar$. This was necessary before we came up with the Huffman trick; I'll go back and change this once we figure out what we're doing with that}

    If for some prompt this probability becomes non-negligible when $f$ is replaced by the PRF, an adversary can break the security of the PRF by running the detection algorithm on this prompt. 
    
    \par{\textbf{Correctness.}} 
    \mir{uses the defn of correctness from sam's email}
    We prove that the scheme is $(2\secpar, L)$-correct in the random oracle model. Let $f$ be a random function.
    Let $x=\Wat_\sk(\prompt)$ be an output of the watermarking procedure such that there exists a subsequence of $x$ of length at most $L$ with empirical entropy at least $2\secpar$.
    In other words, there exists an index $i$ such that $\empH^{[i:i+\ell]}\left(\Model,\prompt,x\right) \geq 2\secpar$ for $\ell = \min\{i+\ell, |x|\}$.
    Note that this is a deterministic property, independent of $\sk$. \sam{To be clear it's not really independent of $\sk$ right? Since $\sk$ influences $x$. but it is a deterministic property of $\prompt,x$.}
    Assume that the tokens used for $r$ use up at most $\secpar$ empirical entropy (we will show how to remove this assumption later). 
    That is, there is an index $j \geq |r|$ for which $\empH^{[j+1:j+\ell]}\left(\Model,\prompt,x\right) \geq \secpar$.
    By \Cref{corollary:watermark-bias-shannon}, 
    \begin{align*}
        \E_{f} \left[\sum_{i=j+1}^{j+\ell}\ln \frac{1}{1-f(r, i, x_i)} \right] &\geq \sum_{i=j+1}^{j+\ell} 1 + 0.9\empH(p_i(x_i))\\
        &= \ell + 0.9 \empH^{[j+1:j+\ell]}\left(\Model,\prompt,x\right)\\
        &\geq \ell + 0.9\secpar
    \end{align*}
    Since each call to $f$ uses a different counter $i$, each term $\ln \frac{1}{1-f(r,i,x_i)}$ in the summation is an independent random variable $X_i$ and we can apply a Chernoff bound.
    Let $\delta$ be the constant such that $(\ell + 0.9\secpar)(1-\delta) = \ell + \frac{\secpar}{2}$; $\delta$ is indeed a constant because $\ell \leq L = c \cdot \secpar$.
    \begin{align*}
        \Pr\left[\sum_{i=j+1}^{j+\ell} X_i \leq \ell + \frac{\secpar}{2}\right] &= \Pr \left[\sum_{i=j+1}^{j+\ell} X_i \leq (\ell + 0.9\secpar)(1 + \delta) \right]\\
        &\leq \exp{\frac{-(\ell + 0.9\secpar)\delta^2}{2}}\\
        &\leq \negl
    \end{align*}
    Therefore, with overwhelming probability, the detection algorithm's count $c_{|r|,j+1}$ will be at least $\frac{\secpar}{2}$, and it will output $\true$.

    Suppose that there exists a prompt $\prompt$ such that with non-negligible probability, $x \gets \Wat_\sk(\prompt)$ has a subsequence of length at most $L$ with empirical entropy at least $2\secpar$.
    If $\Pr[\Detect_\sk(x) = \false]$ is non-negligible when the random oracle is replaced with the PRF, there exists an efficient distinguisher breaking the PRF by sampling $x \gets \Wat_\sk(\prompt)$ and running the detection algorithm.
\end{proof}

==> 99-old-weaker-undetectability.tex <==
\subsection{What does undetectability mean?}
We consider three notions of undetectability. In order of increasing strength, they are:
\begin{itemize}
	\item \emph{Weak undetectability} says that the quality of the output text is not too bad.
	\item \emph{One-shot undetectability} says that a computationally bounded adversary cannot distinguish between the model and the watermarked version using only a single query.
	\item \emph{Strong undetectability} says that a computationally bounded adversary cannot distinguish between the model and the watermarked version using polynomially many queries.
\end{itemize}
We give constructions satisfying all three definitions. For our constructions, there is a trade-off between undetectability and security.


\subsection{Weak undetectability}
\orz{Unnecessary section as we don't care about weak undet, but if we want to have a nice walk-trough we can start with this subsection and call it "planting a signal in a token", to introduce the gumbal thing and just present it as an equivalent construction to KGW/Scott, of planting a signal in a token by "prefering" certain tokens. Next subsection we point out that this is problematic as then you can notice that all tokens are biased in the same way, and thus we should include the index - giving as one-output undet. Finally, we bring up that for multiple outputs we need fresh randomness and then our way of getting it.
Also, none of this should be here in the intro, it should all be a walk-through in the construction section.}

\sam{certainly we should mention that \cite{kgw} considers this sort of thing in the form of ``perplexity'' but we shouldn't dwell on it except to say we don't like it.}

\subsection{One-shot undetectability}
\sam{I'm not sure if I think we should keep this section.}
\orz{All of this is definitely not for the intro}
\begin{definition}[One-Shot Undetectability]
A watermarking scheme $\calW$ is computationally (resp. statistically) \emph{one-shot undetectable} for a model $\Model$ if for all computationally bounded (resp. unbounded) distinguishers $D$ and prompts $\prompt$,
\[\left|\Pr\left[D(A(\prompt), 1^\secpar) = 1\right] - \Pr\left[D(\Model(\prompt), 1^\secpar) = 1 \right]\right| \leq \negl\]
\end{definition}

Let $h : [n] \times \calT \to (0,1)$ be an $(L \cdot \abs{\calT})$-wise independent hash function. Our one-shot undetectable watermarking scheme is:

\begin{algorithm}[H]
\caption{One-shot undetectable scheme.}
\label{alg:one-shot-scheme}
	\KwData{A prompt ($\prompt$)}
	\KwResult{Watermarked text $x_1, \hdots, x_n$}
	$i \gets 0$\;
	\While{$x_i \ne \texttt{done}$}{
		$i \gets i + 1$\;
		$p_i \gets \Model(\prompt, x_1, \hdots, x_{i-1})$\;
		$x_i \gets \argmax\limits_{x \in \calT}\{\log p_i(x) -\log(-\log h(i,x))\}$\;
	}
\end{algorithm}

Given text $x_1, \hdots, x_n$, you can test any set $A \subseteq [n]$ of indices for the watermark against a starting position. More precisely, for any set of indices $A \subseteq [n]$ and (injective) function $\pi : [n] \to [L]$, we can check whether $\{h(\pi(a), x_a)\}_{a \in A}$ is biased towards 1. This could protect against, e.g., the vanilla emoji attack.

\begin{remark}
	\Cref{alg:one-shot-scheme} gives completely deterministic responses, which might be undesirable. If we wanted to simply inject randomness, we could use $h : [n] \times \calT \to \{0,1\}$ and sample the rest of the randomness uniformly instead. This would remain one-shot correct, but since it is slightly less natural, it does not yield any formal improvements in undetectability, it sacrifices some detectability, and strong undetectability necessitates random responses, we focus on the deterministic version of \Cref{alg:one-shot-scheme}.
\end{remark}

